Neuromodulated Learning in Deep Neural Networks

In the brain, learning signals change over time and synaptic location, and are applied based on the learning history at the synapse, in the complex process of neuromodulation. Learning in artificial neural networks, on the other hand, is shaped by hyper-parameters set before learning starts, which remain static throughout learning, and which are uniform for the entire network. In this work, we propose a method of deep artificial neuromodulation which applies the concepts of biological neuromodulation to stochastic gradient descent. Evolved neuromodulatory dynamics modify learning parameters at each layer in a deep neural network over the course of the network's training. We show that the same neuromodulatory dynamics can be applied to different models and can scale to new problems not encountered during evolution. Finally, we examine the evolved neuromodulation, showing that evolution found dynamic, location-specific learning strategies.

==> grn.tex <==
\section{Implementation}
\label{sec:grn}

%% \section{Gene Regulatory Network}

An AGRN is composed of multiple artificial proteins, which interact via evolved
properties. These properties, called tags, are: the protein \emph{identifier},
encoded as a floating point value between 0 and 1; the \emph{enhancer
  identifier}, encoded as a floating point value between 0 and 1, which is used
to calculate the enhancing matching factor between two proteins; the
\emph{inhibitor identifier}, encoded as a floating point value between 0 and 1,
which is used to calculate the inhibiting matching factor between two proteins
and; the \emph{type}, either \emph{input}, \emph{output}, or \emph{regulator},
which is a constant set by the user and is not evolved. 
%SCB:
The identifiers are a representation of 3-D conformations of proteins and enhancing and inhibiting  
%KISH: binding energies?^^^

Each protein has a concentration, representing the use of this protein and
providing state to the network. For \emph{input} proteins, the concentration is
given by the environment and is unaffected by other proteins. \emph{output}
protein concentrations are used to determine actions in the environment; these
proteins do not affect others in the network. The bulk of the computation is
performed by \emph{regulatory} proteins, an internal protein whose concentration
is influenced by other \emph{input} and \emph{regulatory} proteins.

We will first present the classic computation of the GRN dynamics, using
equations found to be optimal in \cite{disset2017comparison} on a number of
problems. Following this overview, we will present the conversion of these
equations into a set of differentiable matrix operations.

The dynamics of the GRN are calculated as follows. First, the absolute affinity of a
protein $a$ with another protein $b$ is given by the enhancing factor
$u^{+}_{ab}$ and the inhibiting $u^{-}_{ab}$:
\begin{equation}
\label{eq:affinity_first}
u^{+}_{ij}=u_{size}-|enh_j-id_i|~~;~~u^{-}_{ij}=u_{size}-|inh_j-id_i|
\end{equation}

where $id_x$ is the identifier, $enh_x$ is the enhancer identifier and $inh_x$
is the inhibitor identifier of protein $x$. The maximum enhancing and inhibiting
affinities between all protein pairs are determined and are used to calculate
the relative affinity, which is here simply called the affinity:
\begin{equation}
\label{eq:affinity_main}
A^{+}_{ij}=-\beta u^{+}_{ij}~~;~~A^{-}_{ij}=-\beta u^{-}_{ij}
\end{equation}
$\beta$ is one of two control parameters used in a GRN, both of which are
described below.

These affinities are used to then calculate the enhancing and inhibiting
influence of each protein, following
\begin{equation}
\label{eq:dynamics_1}
g_i=\frac{1}{N}\sum_j^N{c_je^{A^{+}_{ij}}}~~;~~h_i=\frac{1}{N}\sum_j^N{c_je^{A^{-}_{ij}}}
\end{equation}
where $g_i$ (resp. $h_i$) is the enhancing (resp. inhibiting) value for a
protein $i$, $N$ is the number of proteins in the network, $c_j$ is the
concentration of protein $j$.

The final modification of protein $i$ concentration is given by the following
differential equation:
\begin{equation}
\label{eq:dynamics_2}
\frac{dc_i}{dt}=\frac{\delta(g_i-h_i)}{\Phi}
\end{equation}
where $\Phi$ is a function that normalizes the output and regulatory protein
concentrations to sum to 1.

$\beta$ and $\delta$ are two constants that determine the speed of reaction of
the regulatory network. The higher these values, the more sudden the transitions
in the GRN. The lower they are, the smoother the transitions. In this work, the
$\beta$ and $\delta$ parameters are both evolved as a part of the GRN chromosome
and learned in the optimization of the differentiable GRN.

\section{Differentiable GRN}

%% In TensorFlow, a set of functions with defined gradients, Tensors, can be
%% composed into a differentiable function graph. TensorFlow is also optimized to
%% handle large matrix operations. It was therefore necessary to convert the above
%% computations into Tensors using the functions defined in TensorFlow, and
%% beneficial to convert them into matrix operations.

In this representation of the GRN, protein tags are separated into three vectors
based on their function, $\vec{id}$, identifier, $\vec{enh}$, enhancer, and
$\vec{inh}$, inhibitor. This is their form in evolution and the evolved vectors
serve as initial values for learning. Protein concentrations are also
represented as a vector, following the same indexing as the protein tags.
Initial value for protein concentrations is 0.

%% \begin{gather}
%% \vec{id} = [id_0, id_1, \cdots, id_N]\\
%% \vec{enh} = [enh_0, enh_1, \cdots, enh_N]\\
%% \vec{inh} = [inh_0, inh_1, \cdots, inh_N]\\
%% \vec{c} = [c_0, c_1, \cdots, c_N]
%% \end{gather}

%% The ordering of the proteins is first the $n\_input$ input proteins followed by
%% $n\_output$ output proteins and then finally $n\_regulatory$ regulatory
%% proteins. $n\_input$ and $n\_output$ are based on the environment in which the
%% GRN is used, and $n\_regulatory$ is decided by evolution.

%% The protein tags are then tiled to create three matrices. The enhancing and
%% inhibiting matrices are transposed, resulting in the following:

%% \begin{gather}
%% ID =
%% \begin{pmatrix}
%%   id_0 & id_1 & \cdots & id_N\\
%%   \vdots  & \vdots  & \ddots & \vdots  \\
%%   id_0 & id_1 & \cdots & id_N\\
%% \end{pmatrix}\\
%% ENH =
%% \begin{pmatrix}
%%   enh_0 & enh_0 & \cdots & enh_0\\
%%   \vdots  & \vdots  & \ddots & \vdots  \\
%%   enh_N & enh_N & \cdots & enh_N\\
%% \end{pmatrix}\\
%% INH =
%% \begin{pmatrix}
%%   inh_0 & inh_0 & \cdots & inh_0\\
%%   \vdots  & \vdots  & \ddots & \vdots  \\
%%   inh_N & inh_N & \cdots & inh_N\\
%% \end{pmatrix}
%% \end{gather}

The protein tags are then tiled to create three matrices. The enhancing and
inhibiting matrices are transposed, and the affinities are then calculated for
each element of the matrix using broadcasting, to be expressed in the form of
the net influence of a protein on another protein, referred to as the protein
signatures, $S$:

\begin{gather}
A^{+} = -\beta |ENH - ID|~~;~~A^{-} = -\beta |INH - ID|~~;~~\\
S = e^{A^{+}}-e^{A^{-}}
\end{gather}

The protein tags $\vec{id}, \vec{enh}, \vec{inh}$ are all optimized by learning,
as well as the $\beta$ and $\delta$ GRN parameters. The protein tags are
constrained during optimization to be in $[0.0, 1.0]$, and $\beta$ and $\delta$
are constrained between the parameter values $[\beta_{min}, \beta_{max}]$ and
$[\delta_{min}, \delta_{max}]$, which, for this run, were both $[0.05, 2.0]$.
Learning therefore directly augments evolutionary search in this work; evolution
also optimizes the protein tags, $\beta$, and $\delta$, and is bound by the same
constraints.

\section{GRN layer}

The differentiable GRN model is encoded as a Keras layer to facilitate use.
Keras is a popular deep learning framework which includes many implemented
layers, such as dense, convolutional, and recurrent neural network layers.
Layers are added to a model class, which provides the interface for learning and
evaluation. Here we consider the GRN layer calculation as compared to common
neural network layers, shown in \autoref{fig:grn_layer}. This is not how
the layer is implemented, but is shown rather to demonstrate the difference
between the GRN and existing layer types.

Input proteins influence output and regulatory proteins according to their
respective signatures, which can be considered as weights; the first part of a
GRN layer is therefore like a fully connected layer containing the output
regulatory proteins. These protein concentrations are also influenced by the
previous concentrations of the regulatory proteins, where the signatures from
the regulatory proteins act as weights to all non-input proteins. Output
proteins, however, do not influence regulatory proteins. The layer is therefore
similar to a classic recurrent layer, in that nodes have non-zero weights
between each other depending on their previous activation, but the state of this
layer is stored in the regulatory proteins alone, not in the output proteins.

Finally, a large difference between a recurrent layer and the GRN is the
normalization function, which can be modeled as a softmax layer. It is important
to note that the softmax layer is applied before saving the state of the layer;
the regulatory protein concentration which affects the next time-step is already
normalized. Normalization has been shown to be an important part of artificial
GRN evolution and use \cite{disset2017comparison}, however it may confound deep
neural models not accustomed to having a softmax in the interior of the model.
In \autoref{fig:grn_layer_no_norm}, a GRN layer with no normalization is
considered.

Without normalization, the GRN layer resembles a classic recurrent layer
containing the regulatory proteins followed by a fully connected layer
containing the output proteins. However, as input proteins directly influence
output proteins, there must be connections from the inputs to the fully
connected output layer as well.

With these architectural comparisons in mind, the GRN layer resembles common
neural network functions. Proteins behave as rectified linear units, as they are
bound by 0 but otherwise apply no activation transformation. Unlike artificial
neurons, however, GRN proteins have no bias; the activation is simply the sum of
the weighted input. Finally, it is important to note that, while the signature
matrix can be used to represent weights between nodes, the signature matrix was
not optimized during training. Rather, the protein tags $\vec{id}, \vec{enh},
\vec{inh}$ are optimized by learning, as well as the $\beta$ and $\delta$ GRN
parameters. The training is therefore constrained, similar to how convolutional
layers use a kernel to represent multiple weights.

%% Next, the signatures must be used to determine changes in protein
%% concentrations. Input proteins take concentration values from the environment
%% and influence regulatory and output protein concentrations. Output proteins,
%% however, do not influence other proteins; a mask is therefore applied during the
%% protein concentration update. This mask is composed of 1s for input proteins, 0s
%% for output proteins, and 1s for hidden proteins. Masked concentration values are
%% then multiplied by the signature matrix to determine the change in
%% concentration. Finally, concentrations are normalized.
%% \begin{gather}
%% \vec{mask} = [1, 1, \cdots, 0, 0, 0, \cdots, 1]\\
%% %% \vec{c}[c_0, \cdots, c_{n\_input}] = \texttt{environment\_input()}\\
%% \vec{c_i} = input_i ~~ \forall ~~ i \in [0, n_{input}]\\
%% \vec{c_{mask}} = \vec{c} \odot \vec{mask}\\
%% \vec{\Delta c} = \frac{\delta}{N}\vec{c_{mask}} S\\
%% \vec{c'} = \vec{c} + \vec{\Delta c}\\
%% \vec{c'} = \frac{\vec{c'}}{\sum_{i=n_{input}}^N \vec{c'_i}}
%% \end{gather}

%% The specification of functions in this format is important to ensure
%% compatibility with predefined Tensors, allowing for differentiability. We
%% encourage interested readers to examine the source code repository for more
%% detail on how the GRN Tensor graph is created.

%% \section{Learning}

%% This differentiable GRN model is incorporated into a Keras layer to facilitate
%% use. Keras is a popular deep learning framework which includes many implemented
%% layers, such as dense, convolutional, and recurrent neural network layers.
%% Layers are added to a model class, which provides the interface for learning and
%% evaluation. Two different GRN layer types are used in this work; a one-shot
%% layer and a recurrent layer.

%% In the one-shot, or simple, layer, each data sample is fed into the model,
%% setting the input protein concentrations to the data values. The GRN is stepped
%% once, calculating the concentrations based on the input concentrations once, and
%% the output protein concentrations are returned. This operation is repeated for
%% each data point.

%% The recurrent layer is intended for time-series data. In this layer, data must
%% be pre-configured such that each data sample represents a window of multiple,
%% $w$ samples. Each sample is then fed into the GRN layer in order over the length
%% of window, $w$, and the GRN is stepped after each sample. Finally, the output of
%% the GRN is returned after the last sample. This functionality is identical to
%% that of stateless Recurrent Neural Network (RNN) layers in Keras and is intended
%% to be familiar to users of the library.

%% In both layer types, an error function can be defined using the GRN output and
%% data labels. The error function can be determined by the user with the Keras
%% model interface. The optimization method can also be chosen using this
%% interface. In this work, the Adam optimizer was used, which is a form of
%% stochastic gradient descent that automatically adjusts the learning rate
%% \cite{kingma2014adam}.

%% The protein tags $\vec{id}, \vec{enh}, \vec{inh}$ are all optimized by learning,
%% as well as the $\beta$ and $\delta$ GRN parameters. The protein tags are
%% constrained during optimization to be in $[0.0, 1.0]$, and $\beta$ and $\delta$
%% are constrained between the parameter values $[\beta_{min}, \beta_{max}]$ and
%% $[\delta_{min}, \delta_{max}]$, which, for this run, were both $[0.05, 2.0]$.
%% Learning therefore directly augments evolutionary search in this work; evolution
%% also optimizes the protein tags, $\beta$, and $\delta$, and is bound by the same
%% constraints.

\section{Evolution}

The evolutionary method used in this work is the Gene Regulatory Network
Evolution Through Augmenting Topologies (GRNEAT) algorithm
\cite{Cussat-Blanc2015a}. GRNEAT is a specialized Genetic Algorithm for GRNs
which uses an initialization of small networks, speciation to limit competition
to similar individuals, and a specialized crossover which aligns parent genes
based on a protein distance when creating the child genome. It has been shown to
improve results over a standard GA when evolving GRNs on a variety of tasks.

